Conic Blackwell Algorithm: Parameter-Free Convex-Concave Saddle-Point Solving

We develop new parameter-free and scale-free algorithms for solving convex-concave saddle-point problems. Our results are based on a new simple regret minimizer, the Conic Blackwell Algorithm$^+$ (CBA$^+$), which attains $O(1/\sqrt{T})$ average regret. Intuitively, our approach generalizes to other decision sets of interest ideas from the Counterfactual Regret minimization (CFR$^+$) algorithm, which has very strong practical performance for solving sequential games on simplexes. We show how to implement CBA$^+$ for the simplex, $\ell_{p}$ norm balls, and ellipsoidal confidence regions in the simplex, and we present numerical experiments for solving matrix games and distributionally robust optimization problems. Our empirical results show that CBA$^+$ is a simple algorithm that outperforms state-of-the-art methods on synthetic data and real data instances, without the need for any choice of step sizes or other algorithmic parameters.

==> text/intro__Julien_Grand-Cle__ment_s_conflicted_copy_2021-10-07_.tex <==

\section{Introduction}
\label{sec:intro}

We are interested in solving \emph{saddle-point problems} (SPPs) of the form
\begin{align}\label{eq:spp}
\min_{\bm{x} \in \XX}  \max_{\bm{y} \in \YY} F(\bm{x},\bm{y}),
\end{align}
where $\XX \subset \R^{n}, \YY \subset \R^{m}$ are convex, compact sets, and $F: \XX \times \YY \rightarrow \R$ is a differentiable convex-concave function.
Convex-concave SPPs arise in a number of practical problems. For example, the problem of computing a Nash equilibrium of a zero-sum games can be formulated as a convex-concave SPP, and this is the foundation of most methods for solving sequential zero-sum games~\citep{stengel1996efficient,zinkevich2007regret,tammelin2015solving,kroer2018faster}. They also arise in imaging~\citep{ChambollePock2011}, $\ell_{\infty}$-regression \cite{sidford2018coordinate}, Markov Decision Processes \cite{Iyengar,Kuhn,sidford2018coordinate}, and in distributionally robust optimization, where the max term represents the distributional uncertainty~\citep{namkoong2016stochastic,ben2015oracle}. In this paper we propose efficient, \textit{parameter-free} algorithms for solving \eqref{eq:spp} in many settings, i.e., algorithms that do not require any tuning or choices of step sizes.

\paragraph{Repeated game framework}
One way to solve convex-concave SPPs is by viewing the SPP as a repeated game between two players, where each step $t$ consists of one player choosing $\bm{x}_t\in \XX$, the other player choosing $\bm{y}_t\in \YY$, and then the players observe the payoff $F(\bm{x}_t,\bm{y}_t)$.
If each player employs a regret-minimization algorithm, then a well-known folk theorem says that the uniform average strategy generated by two regret minimizers repeatedly playing an SPP against each other converges to a solution to the SPP.
We will call this the ``repeated game framework.''

There are already well-known algorithms for instantiating the above repeated game framework for \eqref{eq:spp}. 
For example, one can employ the \emph{online mirror descent} algorithm, which generates iterates as follows for the first player (and similarly for the second player):
\begin{align}\label{eq:omd}
       \bm x_{t+1} = \argmin_{\bm x \in \XX} \langle \eta \nabla_{\bm{x}} F(\bm{x}_t, \bm{y}_t), \bm{x} \rangle + D(\bm x \| \bm x_{t}),
\end{align}
where $D(\cdot \| \cdot)$ is a Bregman divergence which measures distance between pairs of points and $\eta>0$ is an appropriate step size. By choosing $D$ appropriately for $\XX$, the update step \eqref{eq:omd} becomes efficient, and one can achieve an overall regret on the order of $O(\sqrt{T})$ after $T$ iterations. \tb{This regret can be achieved either by choosing a fixed step size $\eta = \alpha /L \sqrt{T}$, where $L$ is an upper bound  on the norms of the gradients visited $\left( \nabla_{\bm{x}} F(\bm{x}_t, \bm{y}_t) \right)_{t \geq 0}$, or by choosing adaptive step sizes $\eta_{t} = \alpha / \sqrt{t}$, for $\alpha>0$.  This is problematic,  as 1) the upper bound $L$ may be hard to obtain in many applications and may be too conservative in practice, and 2) adequately tuning the parameter $\alpha$ can be time- and resource-consuming, and even practically infeasible for very large instances, since we won't know if the step size will cause a divergence until late in the optimization process.} This is not just a theoretical issue,  as we highlight in our numerical experiments (Section \ref{sec:simu}) and in the appendices (Appendices \ref{app:OMD-etc}).
Similar results and challenges hold for the popular \emph{follow the regularized leader} (FTRL) algorithm (see Appendix \ref{app:OMD-etc}).

\paragraph{Regret Matching}
In this paper, we introduce alternative regret-minimization schemes for instantiating the above framework. 
Our work is motivated by recent advances on solving large-scale zero-sum sequential games. 
In the zero-sum sequential game setting,  $\XX$ and $\YY$ are simplexes, the objective function becomes $F(\bm x, \bm y) = \langle \bm{x},\bm{Ay} \rangle$, and thus \eqref{eq:spp} reduces to a \emph{bilinear} SPP.
Based on this bilinear SPP formulation, the best practical methods for solving large-scale sequential games use the repeated game framework, where each player minimizes regret via some variant of \emph{counterfactual regret minimization} (CFR, \citep{zinkevich2007regret}).
Variants of CFR were used in every recent poker AI challenge, where poker AIs beat human poker players~\citep{bowling2015heads,moravvcik2017deepstack,brown2018superhuman,brown2019superhuman}.
The CFR framework itself is a decomposition of the overall regret of the bilinear SPP into local regrets at each decision point in a sequential game~\citep{farina2019online}.
The key to the practical performance of CFR-based algorithms seems to be three ingredients (beyond the CFR decomposition itself): 
(1) a particular regret minimizer called \emph{regret matching$^+$} (\rmp)~\citep{tammelin2015solving} which is employed at each decision point, 
(2) aggressive iterate averaging schemes that put greater weight on recent iterates (e.g. \emph{linear averaging}, which weights iterate at period $t$ by $2t / T(T+1)$), and 
(3) an alternation scheme where the updates of the repeated game framework are performed in an asymmetric fashion.
The CFR framework itself is specific to sequential bilinear games on simplexes, but these last three ingredients could potentially be generalized to other problems of the form \eqref{eq:spp}.
That is the starting point of the present paper.

The most challenging aspect of generalizing the above ingredients is that \rmp{} is specifically designed for minimizing regret over a simplex. 
However, many problems of the form \eqref{eq:spp} have convex sets $\XX,\YY$ that are not simplexes, e.g. box constraints or norm-balls for distributionally robust optimization~\citep{ben2015oracle}.
In principle, regret matching arises from a general theory called \emph{Blackwell approachability}~\citep{blackwell1956analog,hart2000simple}, and similar constructions can be envisioned for other convex sets.
However, in practice the literature has only focused on developing concrete implementable instantiations of Blackwell approachability for simplexes. 
A notable deviation from this is the work of \citet{abernethy2011blackwell}, who showed a general reduction between regret minimization over general convex compact sets and Blackwell approachability. However, their general reduction still does not yield a practically implementable algorithm: among other things,  their reduction relies on certain black-box projections that are not always efficient.
We show how to implement these necessary projections for the setting where $\XX$ and $\YY$ are simplexes, $\ell_p$ balls, and intersections of the $\ell_2$ ball with a hyperplane (with a focus on the case where an $\ell_2$ ball is intersected with a simplex,  which arises naturally as confidence regions). 
This yields an algorithm which we will refer to as the \emph{conic Blackwell algorithm} (\cba), which is similar in spirit to the regret matching algorithm, but crucially generalizes to other decision sets. Motivated by the practical performance of \rmp{}, we construct a variant of \cba{} which uses a thresholding operation similar to the one employed by {\rmp}. We call this algorithm \cbap{}. 

\paragraph{Our contributions}
We introduce \cbap, a parameter-free algorithm which achieves $O(\sqrt{T})$ regret in the worst case and generalizes the strong performances of \rmp{} for bilinear, simplex saddle-points solving to other more general settings.
%Motivated by the practical performance of \rmp{}, we show how to construct a variant of \cba{} which uses a thresholding operation similar to the one employed by {\rmp}. We call this algorithm \cbap{}. Both \cba{} and \cbap{} achieve $O(\sqrt{T})$ regret in the worst case.
A major selling point for \cbap{} is that it does not require any step size choices. Instead, the algorithm implicitly adjusts to the structure of the domains and losses by being instantiations of Blackwell's approachability algorithm.
After developing the \cbap{} algorithm, we then develop analogues of another crucial components for large-scale game solving. 
In particular, we prove a generalization of the folk theorem for the repeated game framework for solving \eqref{eq:spp}, which allows us to incorporate  polynomial averaging schemes such as linear averaging.
We then show that \cbap{} is compatible with linear averaging on the iterates. This mirrors the case of RM and \rmp{}, where only \rmp{} is compatible with linear averaging on the iterates.
We also show that both \cba{} and \cbap{} are compatible with polynomial averaging when simultaneously performed on the regrets and the iterates.
%The fact that both \cba and \cbap are compatible is somewhat surprising, because in the game-solving setting, it is only \rmp that is compatible with these ideas.
Combining all these ingredients, we arrive at a new class of algorithms for solving convex-concave SPPs. As long as efficient projection operations can be performed (which we show for several practical domains, including the simplex, $\ell_{p}$ balls and confidence regions in the simplex), one can apply the repeated game framework on \eqref{eq:spp}, where one can 
 use either \cba{} or \cbap{} as a regret minimizer for $\XX$ and $\YY$, use polynomial averaging on the generated iterates,  in order to solve \eqref{eq:spp} at a rate of $O \left( 1/\sqrt{T} \right)$.
 
We highlight the practical efficacy of our algorithmic framework on several domains.
First, we solve two-player zero-sum matrix games and extensive form games, where \rmp{} regret minimizer combined with linear averaging and alternation, and CFR$^+$, lead to very strong practical algorithms~\citep{tammelin2015solving}. We find that \cbap{} combined with linear averaging and alternation leads to a comparable performance in terms of the iteration complexity, and may even slightly outperform \rmp{} and CFR$^+$.
Second, we apply our approach to a setting where \rmp{} and CFR$^+$ do not apply: distributionally robust empirical risk minimization (DR-ERM) problems. Across two classes of synthetic problems and four real data sets, we find that our algorithm based on \cbap{} performs orders of magnitude better than online mirror descent and FTRL, as well as their optimistic variants, when using their theoretically-correct fixed step sizes.
%We test the practical efficacy of our algorithmic framework on several domains.
%First, we solve two-player zero-sum matrix games. In this setting, we already know that the \rmp{} regret minimizer combined with linear averaging and alternation leads to a very strong practical algorithm~\citep{tammelin2015solving}. We find that \cbap{} combined with linear averaging and alternation leads to a comparable performance in terms of the iteration complexity. Generally we find that \rmp{} performs slightly better initially, but \cbap{} eventually performs slightly better.
%Second, we apply our approach to a setting where \rmp{} does not apply: distributionally-robust empirical risk minimization (DR-ERM) problems. Across two classes of synthetic problems and four real datasets, we find that our algorithm based on \cbap{} performs orders of magnitude better than online mirror descent and FTRL, as well as their optimistic variants, when using their theoretically-correct stepsizes.
Even when considering adaptive step sizes, or fixed step sizes that are up to $10,000$ larger than those predicted by theory, our \cbap{} algorithm performs better, with only a few cases of comparable performance (at step sizes that lead to divergence for some of the other non-parameter free methods). The fast practical performance of our algorithm, combined with its simplicity and the total lack of step sizes or parameters tuning, suggests that it should be seriously considered as a practical approach for solving  convex-concave SPPs in various settings.

Finally, we make a brief note on accelerated methods. Our algorithms have a rate of convergence towards a saddle point of  $O(1/\sqrt{T})$, similar to OMD and FTRL. 
In theory, it is possible to obtain a faster $O \left( 1/T \right)$ rate of convergence, for example via mirror prox~\citep{nemirovski2004prox} or other primal-dual algorithms~\citep{ChambollePock16}. 
However, our experimental results show that \cbap{} is faster than optimistic variants of FTRL and OMD~\citep{syrgkanis2015fast}, the latter being almost identical to the mirror prox algorithm, and both achieving $O(1/T)$ rate of convergence.
A similar conclusion has been drawn in the context of sequential game solving, where the fastest $O(1/\sqrt{T})$ CFR-based algorithms have better practical performance than the theoretically-superior $O \left( 1/T \right)$-rate methods~\citep{kroer2018faster,kroer2018solving}.

